Impact of Parameter Sparsity on Stochastic Gradient MCMC Methods for Bayesian Deep Learning

Bayesian methods hold significant promise for improving the uncertainty quantification ability and robustness of deep neural network models. Recent research has seen the investigation of a number of approximate Bayesian inference methods for deep neural networks, building on both the variational Bayesian and Markov chain Monte Carlo (MCMC) frameworks. A fundamental issue with MCMC methods is that the improvements they enable are obtained at the expense of increased computation time and model storage costs. In this paper, we investigate the potential of sparse network structures to flexibly trade-off model storage costs and inference run time against predictive performance and uncertainty quantification ability. We use stochastic gradient MCMC methods as the core Bayesian inference method and consider a variety of approaches for selecting sparse network structures. Surprisingly, our results show that certain classes of randomly selected substructures can perform as well as substructures derived from state-of-the-art iterative pruning methods while drastically reducing model training times.

==> checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Please look at the experiments, and conclusions sections.}
  \item Did you describe the limitations of your work?
    \answerYes{Please look at the conclusions section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Since our work looks at examining tradeoffs for Bayesian neural networks under different sparse substructures, and due to its inherent strong empirical nature, we believe that our work doesn't on its own possess the ability to have potentially negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Our code for generating the results in our paper requires a SLURM based GPU cluster, as well as several days of compute, making it practically infeasible to share during the review cycle. However, we do share the code for the C implementation of the MLP200 test time experiment in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All the training details is provided either in the main body or the supplemental material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Unfortunately, since these experiments take a lot of time to run, we couldn't run them multiple times to assess error bars.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We do provide the exact resources used by our paper in the supplemental material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{Since the data sets used are widely popular, and require authors to only cite them, we've cited them as required, but haven't included their license. However, the license information is easily available for anyone interested.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{Any assets in supplemental material is our work only.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> experiments.tex <==
\section{Experiments}

\subsection{Experimental protocols}


 
\subsection{Experiment 1: SGMCMC in sparse neural networks}
In this experiment, we perform an initial analysis of how SGMCMC methods perform on sparse neural networks. The aim of this experiment is to analyze the predictive performance of sparse Bayesian ensembles. We utilize the iterative global pruning technique to first produce a neural network with a sparsity level $p$ (i.e. $p$ proportion of weights remaining). Next, we initialize our SGHMC chain using the generated neural network as the initialization point and run our sampler. Finally, we collect the monte carlo samples and evaluate the predictive performance as shown in the Table  \ref{tab:basic_results}. A brief description of the different results presented in table \ref{tab:basic_results} is given below:

\begin{itemize}
    \item \textbf{Non-sparse model}: This represents the experiment where we do not perform any pruning on the model.
    
    \item \textbf{Sparse - iterative pruning}: This represents the scenario where we iteratively prune the model to a certain sparsity level. Iterative pruning method comprises of multiple training-pruning steps. In our experiments, at every pruning step, we prune 20\% of the remaining unpruned weights globally. Once we execute our pruning step, we re-train the model with the remaining weights. These interleaved steps are repeated until we achieve $p$ sparsity.
    
    \item \textbf{Sparse - LTH}: This represents the scenario where we use the lottery ticket hypothesis (LTH) to obtain sparse sub-networks, which if initialised with the same parameters, lead to a similar level of performance as the non-sparse model. As with iterative pruning, the LTH method comprises of multiple training-pruning steps. However, after every pruning step, we rewind all the remaining parameters to the original initialised version. Once this is done, we re-train the model with the re-winded weights and perform this iteratively until we achieve $p$ sparsity. 
    
    \item \textbf{Random Mask}: This represents the scenario where we apply random masks on the model parameters. In our work, explore 3 different methods of generating these random masks. In the first method, we take an existing mask (either from LTH or iterative pruning experiment), and generate a random mask which has the same sparsity per-layer as that of the existing mask under consideration. In the second method, we pool all the parameters of our model and randomly prune out a set of the parameters to achieve our desired level of sparsity $p$. Finally, in the third method, we randomly prune out $p$ proportion of parameters every layer, so as to achieve a global $p$ sparsity. 
    
    \item \textbf{Chains with random mask(s)}: Building off the random masks described earlier, we perform experiments where we perform a parallel-chain style experiments using SGHMC where each chain represents a random mask generated by either of the random masking approaches described earlier. For comparison, we also present the case where we use a single chain and ensure that the final number of MCMC samples collected are constant for a fair comparison.  
    
\end{itemize}

Some experimental questions to answer in the paper:

\begin{enumerate}
    \item Is there a difference between iterative pruning and lottery ticket? (Compare iterative pruning with lottery ticket)
    \item How dependent are SGHMC on their initialisation? (i.e. start from lottery ticket, start from SGD, start from end of iterative pruning etc...).
    \item We \textbf{must} compare to just a smaller model. (like a dense NN that has the same number of weights as a sparse one).
    \item We are interested in \textbf{what do we do with a certain parameter budget}. I.e. Our parameter budget is $X$, how do we arrange our weights to get the best posterior. 
    \item Comparing training time vs testing time vs sampling time.
    \begin{itemize}
        \item Simple model is fast
        \item Sparse model is cheaper for storage
        \item Subspace inference is expensive
    \end{itemize}
\end{enumerate}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Performance comparison between SGHMC on sparse ($p=0.1$) and non-sparse networks. SGD baselines are also given for reference. This is using ResNet18 and CIFAR10.}
\label{tab:basic_results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ccc}
\toprule
SGD (non-sparse)   & 0.45 & 90.58\%  \\ \midrule
SGD (sparse, iterative pruning)       & 0.44 & 89.05\%   \\ \midrule
SGD (sparse, iterative pruning, random mask)       & 0.48 & 84.0\%   \\ \midrule
SGHMC (non-sparse) & 0.22 & 92.57\%  \\ \midrule
SGHMC (sparse, iterative pruning)     & 0.28 & 90.69\% \\ \midrule
SGD (sparse, LTH) & 0.50 & 90.25 \% \\ \midrule
SGD (sparse, LTH, random mask)       & 0.388 & 90.01\%   \\ \midrule
SGHMC (sparse, LTH) & 0.32 & 91.13 \% \\ \midrule
SGHMC (sparse, pretrained LTH) & 0.2777 & 92.83 \% \\ \midrule
SGHMC (sparse, LTH, random masks, 5 chains, 10 samples each) & 0.2121 & 93.53 \% \\ \midrule
SGHMC (sparse, LTH, random masks, 1 chain, 50 samples) & 0.2625 & 92.54 \% \\ \midrule
SGHMC (sparse, iterative pruning, random masks, 1 chain, 50 samples) & 0.2657 & 92.61 \% \\ \midrule
SGHMC (sparse, iterative pruning, random masks, 5 chains, 10 samples each) & 0.2122 & 93.57 \% \\ \midrule
SGHMC (sparse, 10\% layer-by-layer, 1 chains, 50 samples each) & 0.2763 & 91.61 \% \\ \midrule
SGD (sparse, 10\% layer-by-layer) & 0.41 & 90.69 \% \\
\bottomrule
\end{tabular}%
% }
\end{table*}

\begin{table*}[]
\small
\centering
\caption{Fashion MNIST MLP200. Comment: This was sensitive to hyperparameters but these hyperparameters get very good performance! SGHMC looks like it might be struggling (to mix?) in the very low sparsity networks.}
\label{tab:basic_results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
Pruned &\multicolumn{2}{c}{(0 \%)} & \multicolumn{2}{c}{(89.1 \%)}& \multicolumn{2}{c}{(94.3 \%)} & \multicolumn{2}{c}{(98.4 \%)} & \multicolumn{2}{c}{(99.3 \%)} \\
                  & NLL  & Acc. & NLL  & Acc. & NLL  & Acc. & NLL  & Acc. \\ \midrule
SGD (LTH) & 0.298 & 89.79 & 0.316 & 89.61 & 0.315 & 89.48 & 0.320 & 88.77 & 0.379 & 86.39 \\
SGD (IP) & 0.298 & 89.79 & 0.338 & 89.67 & 0.338 & 89.44 & 0.318 & 88.85 & 0.367 & 86.95 \\
SGD (Rand. Mask, global) & 0.298 & 89.79 & 0.360 & 87.19 & 0.406 & 85.09 & 0.813 & 72.08 & 2.149 & 16.38 \\\midrule
\multicolumn{11}{c}{50 Burn, 50 Samples. (Run 1, with no pre-train, Run 2 with pre-train)} \\
SGHMC (LTH, Run 1) & 0.280 & 90.29 & 0.302 & 89.52 & 0.306 & 89.33 & 0.338 & 88.06 & 0.425 & 84.84  \\
SGHMC (LTH, Run 2) & 0.281 & 90.17 & 0.310 & 89.40 & 0.311 & 89.40 & 0.318 & 88.79 & 0.374 & 86.71  \\
\bottomrule
\end{tabular}%
% }
\end{table*}

\begin{table*}[]
\small
\centering
\caption{Mean effective sample size. The same random mask must be used for all chains here for a fair application of the ESS across the chains. This is over the 50 samples post burn-in. FMNIST}
\label{tab:basic_results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Pruned &0 \% & 89.1 \%& 95.3 \% \\
SGHMC (LTH, 5 Chains) & 3.1969 & 4.6081 & 5.7829\\
SGHMC (Random Mask LTH Proportion, 5 Chains) & - & 2.6937 & 2.7511\\
SGHMC (Layer-wise Random Mask, 5 Chains) & - & 3.0512 & 3.6698\\
SGHMC (Global Random Mask, 5 Chains) & - & 3.1178 & 3.5895\\
\bottomrule
\end{tabular}%
% }
\end{table*}

% # ESS LTH 0 10 chains #11.6477, # 5 chains 6.4508
% #        10 10 chains #15.4836, # 5 chains 8.4667
% #        14 10 chains #18.7471, # 5 chains 10.1034

\begin{table*}[]
\small
\centering
\caption{ResNet20}
\label{tab:basic_results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Pruned &\multicolumn{2}{c}{(0 \%)} & \multicolumn{2}{c}{(89.0 \%)}& \multicolumn{2}{c}{(95.3 \%)} \\
                  & NLL  & Acc. & NLL  & Acc. & NLL  & Acc.  \\ \midrule
SGD CIFAR10 (LTH) & 0.430 & 89.28 & 0.400 & 89.10 & 0.408 & 86.83 \\
SGHMC CIFAR10 (LTH) & 0.295 & 91.23 & 0.33656 & 89.39 & 0.3737 & 87.39  \\
SGHMC CIFAR10 - 5 chains (LTH) & TBA & TBA & 0.3607 & 0.8965 &  0.382 & 87.45  \\
SGHMC CIFAR10 (IP) & 0.295 & 91.23 & 0.3656  & 87.69 & 0.3294 &   89.82\\
SGHMC CIFAR10 - 5 chains (IP) & TBA & TBA & 0.3625  & 89.62 & 0.3761 & 87.6\\
SGD CIFAR10 (IP) & 0.424 & 89.67 & 0.416 & 89.43 & 0.398 & 87.55 \\\midrule
SGD CIFAR100 (LTH) & 1.37 & 67.55 & 1.59 & 56.46 & 1.97 & 47.72 \\
SGD CIFAR100 (IP) & 1.41 & 67.36 & 1.32 & 65.05 & 1.53 & 58.08\\
\bottomrule
\end{tabular}%
% }
\end{table*}

% # 0: 0.2810 #10 0.3097 #13 0.3112  #19 0.3180 24 0.3744
% #0: 0.9017 #10 0.894 #13 .894 # 19 0.8879 # 24 0.8671

% \begin{table}[]
% \centering
% \caption{MNIST MLP200.}
% \label{tab:basic_results}
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{Fashion MNIST} \\
%                   & NLL  & Accuracy & NLL  & Accuracy \\ \midrule
% SGD (non-sparse)                  & 0.056 & 98.43\% & 0.320 & 88.83\% \\ \midrule
% SGD (sparse, iterative pruning (10.7 \%))   & 0.101 & 97.46\% & 0.421 & 85.71\% \\ \midrule
% SGD (sparse, lottery ticket (10.7 \%))   & 0.092 & 97.35\% & 0.563 & 80.07\% \\ \midrule
% SGD (non-sparse, small model, 35-35 units)     & 0.112 & 96.93\% \\\midrule
% SGD (sparse, 10\% layer-by-layer) & & & 0.393 & 86.05 \% \\
% \midrule
% SGD (sparse, 10\% overall random) & & & 0.352 & 87.65 \% \\
% \midrule
% SGHMC (non-sparse) & 0.059 & 98.44\% & 0.296 & 89.86\%  \\ \midrule
% SGHMC (sparse, 100 samples from iterative pruning)     & 0.097 & 97.50\% & 0.383 & 87.03\% \\ \midrule
% SGHMC (sparse, from lottery ticket sparse (50 burn SGHMC)) & 0.085 & 97.41\% & 0.582 & 79.66\% \\ \midrule
% SGHMC (non-sparse, small model)     & 0.113 & 97.16\% \\\midrule
% SGHMC (sparse, 10\% layer-by-layer, 1 chains, 100 samples each) & & & 0.353 & 87.57 \% \\ \midrule
% SGHMC (sparse, random 10\% full model, 1 chains, 100 samples) & & & 0.347 & 87.74 \% \\ \midrule
% \bottomrule
% \end{tabular}%
% % }
% \end{table}


\subsection{Experiment 2: Effect of mask structures \& initialization on approximate inference}

\subsection{Experiment 3: Analyzing storage-performance tradeoff of sparse Bayesian ensembles}

\subsection{Experiment 4: Uncertainty quantification using sparse Bayesian ensembles}

\subsection{Experiment 5: Mixing performance comparison between sparse and full models}

We will how using ACF/ESS compares across model paradigms. We could also look a KS statistic between two halves of the chain to see if they converge (using the predictive distribution/entropy as a value). 

\paragraph{Note on KS statistic.} We just subsample to correct for correlation and calculate the KS statistic over two halves of the data. For multiple dimensions, either compute for each parameter of for the function of interest h(). The problem is that the correction for correlation is not guaranteed. However, for comparing inference schemes it could be useful, as each inference scheme uses the same thinning.

We could also look at CUMSUM by plotting for all inference schemes:
$$D_S^i = \frac{1}{S} \sum^i [h(\boldsymbol{\omega}_s) - S_S], \quad \text{where } S_S = \frac{1}{S} \sum h(\boldsymbol{\omega}_s) \text{ and } i = 1, \dots, T$$
When mixing of the chain is high - the graph of $D^i_S$ is highly irregular and concentrated around zero. Slowly mixing chains (already in stationary dist.) produce regular graphs with long excursions away from 0. Page 482 Robert and Casella.


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{instantaneous_NLL_ACF_FMNIST_after_burn.pdf}
\caption{Comparison of the ACF across different sparsity levels, using different masking approaches. The ACF of the instantaneous NLL is computed over the last 50 samples of each method after a burn-in of 50 epochs. The mean and standard deviations are plotted in the figure. Both sparse sub-networks that were derived via the LTH have autocorrelations that drop to zero from lag one onward. In addition, the lower sparsity models ($89.1\ \%$) are also zero at all lags. The high sparsity sub-networks ($95.3\ \%$) that were derived via either of the randomly drawn masks have a slightly higher ACFs that may indicate the challenge of sampling from those subnetworks. These results can further be seen in Figure \ref{fig:inst_nll}, where the sparser networks with randomly drawn masks take longer to plateau.}
\label{fig:acf_nll}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{instantaneous_NLL.pdf}
\caption{This shows how the instantaneous NLL is changing. LTH masks seem to allow for faster convergence.}
\label{fig:inst_nll}
\end{figure}


==> figures/table_exp1.tex <==
\begin{tabular}{llrrl}
\toprule
  Dataset &      Method &     Acc &     NLL &     ECE \\
\midrule
   FMNIST &  Full-SGHMC &  0.9290 &  0.2810 &  0.0084 \\
   FMNIST &    Full-OPT &  0.8979 &  0.2980 &  0.0230 \\\hline
  CIFAR10 &  Full-SGHMC &  0.9113 &  0.2797 &  0.0476 \\
  CIFAR10 &    Full-OPT &  0.8967 &  0.4240 &  0.0610 \\\hline
 CIFAR100 &  Full-SGHMC &  0.6805 &  1.2660 &  0.0325 \\
 CIFAR100 &    Full-OPT &  0.6755 &  1.3700 &  0.1369 \\
\bottomrule
\end{tabular}


==> figures/table_exp3b-1.tex <==
\begin{tabular}{llr}
\toprule
          Method & Sparsity &  Total Time (s) \\
\midrule
        Full-OPT &       0\% &          1811.2 \\
      Full-SGHMC &       0\% &          2943.2 \\
        IP-SGHMC &      83\% &         19244.0 \\
        IP-SGHMC &      89\% &         22866.4 \\
        IP-SGHMC &      95\% &         30111.2 \\
 RLM(F)-SGHMC(1) &      83\% &          2943.2 \\
 RLM(F)-SGHMC(1) &      89\% &          2943.2 \\
 RLM(F)-SGHMC(1) &      95\% &          2943.2 \\
\bottomrule
\end{tabular}


==> figures/table_exp3b-10.tex <==
\begin{tabular}{llr}
\toprule
           Method & Sparsity &  Total Time (s) \\
\midrule
         Full-OPT &       0\% &          1811.2 \\
       Full-SGHMC &       0\% &          2943.2 \\
         IP-SGHMC &      83\% &         19244.0 \\
         IP-SGHMC &      89\% &         22866.4 \\
         IP-SGHMC &      95\% &         30111.2 \\
 RLM(F)-SGHMC(10) &      83\% &         24338.0 \\
 RLM(F)-SGHMC(10) &      89\% &         24338.0 \\
 RLM(F)-SGHMC(10) &      95\% &         24338.0 \\
\bottomrule
\end{tabular}


==> figures/table_exp3b-5.tex <==
\begin{tabular}{llr}
\toprule
          Method & Sparsity &  Total Time (s) \\
\midrule
        Full-OPT &       0\% &          1811.2 \\
      Full-SGHMC &       0\% &          2943.2 \\
        IP-SGHMC &      83\% &         19244.0 \\
        IP-SGHMC &      89\% &         22866.4 \\
        IP-SGHMC &      95\% &         30111.2 \\
 RLM(F)-SGHMC(5) &      83\% &         12452.0 \\
 RLM(F)-SGHMC(5) &      89\% &         12452.0 \\
 RLM(F)-SGHMC(5) &      95\% &         12452.0 \\
\bottomrule
\end{tabular}


==> old_main.tex <==
\section{Introduction}
\textbf{Possible objectives:}
\begin{enumerate}
    \item Do sparse models mix better or worse than full models with SGMCMC approaches?
    \item In terms of computational resources, is it better to work with sparse models when performing inference or just do inference in the full networks.
\end{enumerate}


\section{Relevant literature}
% List some papers here:
Lottery ticket codebase: \url{https://github.com/facebookresearch/open_lth }

\section{TO DO list:}
\begin{itemize}
    \item Analyse Log-likelihoods as networks get sparser - how does UQ performance change
    \begin{itemize}
        \item Look at the LL for the original model (both the ensemble with SGHMC and the single SGD model)
        \item Run SGHMC on top of above SGD model and also compare.
        \item These will be compared with the performance of sparse SGD and sparse SGHMC from the lottery ticket inititialisation. (SGD - LL: 0.44, Acc:  after iterative pruning, 10 \% weights remaining; Pretrained sparse SGD + SGHMC tuning - LL: 0.28, ACC:  )
    \end{itemize}
    \item Analyse the effective sample size/autocorrelation function of the samples:
    \begin{itemize}
        \item Does the ESS increase with sparser networks?
        \item Does the ACF drop faster in sparser networks?
    \end{itemize}
    \item Run lottery ticket hypothesis on smaller networks as it might be easier to analyse.
    \item Get the group L1/L2 sparsity working in a notebook.
    \item Parallel chain SGHMC, each chain starts with a different mask structure. Examine these techniques for UQ tasks. (Adversarial attack code).
\end{itemize}

\section{Paper Plan:}

\subsection{Abstract}
In this work, we are interested in how inference works in sparse networks. In our work we will analyse how sparse networks perform compared to both their full (base) models and ensembles of models. We further compare to other approaches that aim to reduce the parameter size in Bayesian inference for neural networks. In particular, we will compare to subspace inference, which aims to reduce the cost of sampling in the large parameter space, by transforming to a lower dimensional subspace. Table \ref{tab:comp} shows structure of how we intend to make such comparisons.

Ideas:
\begin{enumerate}
    \item How do SGMCMC methods compare on sparse structures vs. full structures?
    \begin{itemize}
        \item Mixing
        \item Performance on downstream tasks
        \item Storage trade-off $\rightarrow$ Exploit this trade-off.
    \end{itemize}
    \item Choosing random mask structures and combining samples from different chains with different masks. 
    \item 
\end{enumerate}



\subsection{Convergence:}
The key questions made apparent by this table is how to measure these differences. We need to demonstrate using ACF/ESS how mixing compares across model paradigms. Furthermore, we need to measure convergence to the posterior distribution in terms of resources/time taken. We must also compare the memory costs. We could also look a KS statistic between two halves of the chain to see if they converge (using the predictive distribution/entropy as a value). We just subsample to correct for correlation and calculate the KS statistic over two halves of the data. For multiple dimensions, either compute for each parameter of for the function of interest h(). The problem is that the correction for correlation is not guaranteed. However, for comparing inference schemes it could be useful, as each inference scheme uses the same thinning.

We could also look at CUMSUM by plotting for all inference schemes:
$$D_S^i = \frac{1}{S} \sum^i [h(\boldsymbol{\omega}_s) - S_S], \quad \text{where } S_S = \frac{1}{S} \sum h(\boldsymbol{\omega}_s) \text{ and } i = 1, \dots, T$$
When mixing of the chain is high - the graph of $D^i_S$ is highly irregular and concentrated around zero. Slowly mixing chains (already in stationary dist.) produce regular graphs with long excursions away from 0. Page 482 Robert and Casella.

\begin{table}[h]
\small
    \centering
    \begin{tabular}{c|c|c|c}
         Paradigms & \shortstack{Is inference easier \\ (mixing etc...)}  & \shortstack{Is inference faster \\ (Train vs. Test)} & \shortstack{Memory requirements \\ (Train vs. Test)}\\
         \hline
         Base Model (SGD) &ResNet18 &  & \\
         Base Model (SGHMC) & ResNet18 & &\\
         Smaller Base Model (SGD) & ResNet18 & &\\
         Smaller Base Model (SGHMC) & ResNet18 & &\\
         Parameter-Space Transformation & & &\\
    \end{tabular}
    \caption{Caption}\label{tab:comp}
\end{table}

\begin{figure}
\centering
\includegraphics[height=5.2cm]{ACF.png}
\caption{The ACF of five different weights of the network. Notice how the green weight has very high autocorrelation across the samples.}
\label{fig:acf}
\end{figure}

\section{Experiments}
Experiments that we need run to do comparisons:
\begin{itemize}
    \item 
\end{itemize}




\section{Extensions}

It would be also interesting to investigate whether using lookup tables with a single mask can reduce the storage costs significantly. Especially if we can introduce shared weights that do not vary across samples (we could look to the ACF for potentially lossless compression). 


Looking at multiple masks of similar structure. I.e. an ensemble of different sparse NNs. Can we even learn the sparse structure in the future by using BO over some mask/dropout distribution?

